Long-Term Client Selection for Federated Learning with Non-IID Data: A Truthful Auction Approach

Federated learning (FL) provides a decentralized framework that enables universal model training through collaborative efforts on mobile nodes, such as smart vehicles in the Internet of Vehicles (IoV). Each smart vehicle acts as a mobile client, contributing to the process without uploading local data. This method leverages non-independent and identically distributed (non-IID) training data from different vehicles, influenced by various driving patterns and environmental conditions, which can significantly impact model convergence and accuracy. Although client selection can be a feasible solution for non-IID issues, it faces challenges related to selection metrics. Traditional metrics evaluate client data quality independently per round and require client selection after all clients complete local training, leading to resource wastage from unused training results. In the IoV context, where vehicles have limited connectivity and computational resources, information asymmetry in client selection risks clients submitting false information, potentially making the selection ineffective. To tackle these challenges, we propose a novel Long-term Client-Selection Federated Learning based on Truthful Auction (LCSFLA). This scheme maximizes social welfare with consideration of long-term data quality using a new assessment mechanism and energy costs, and the advised auction mechanism with a deposit requirement incentivizes client participation and ensures information truthfulness. We theoretically prove the incentive compatibility and individual rationality of the advised incentive mechanism. Experimental results on various datasets, including those from IoV scenarios, demonstrate its effectiveness in mitigating performance degradation caused by non-IID data.

==> 7.notation.tex <==
\begin{notation}[ll]
	$A_z^t, a_m$                  & 数据类别内的差异比率       \\
	$B_m^t$                  & 带宽        \\
    $c_{m}^t$             & 数据质量        \\
	$\mathcal{D}_m,{D}_m, d_{z, m}, d_\text{avg}$ & 本地数据集，数据集大小，类别数据大小，类别数据大小平均值       \\
    $E_{m}^\text{cmp}, E_{m}^{t, \text{com}}$ & 计算能耗，通信能耗        \\
    $f_{m}^t$                  & CPU工作频率        \\
	$\textbf{g}^t, {g}_z^t$ & 已学习数据量向量, 已学习数据量\\
    $\hat{h}m$                  & 信道增益        \\
	$\mathcal{I}_{\mathbf{M}-m}$ & 除移动客户端 $m$之外的客户端集合     \\
    $d_\text{max}$                  & 坐标        \\
	$l_m^t$                  &  本地迭代次数       \\
    $\textbf{M}$                  & 移动客户端集合        \\
	$N$                  & 每轮选择的客户端数目       \\
    $\textbf{o}^t$                  & 数据类别差异向量        \\
	$, P$                  & ，通信功率     \\
    ${q}_{m}^t$                  & 赢者指示参数        \\
	$r_m$                  & 奖励 \\
    $s^t$                  & 上行传输速率        \\
	$t$                  & 通信回合        \\
    $u_{z, m}^t, u^\text{c}_m$                 & 数据类别增益，数据多样性增益 \\
    $U_{m}^t, U_\text{s}^t, U_\text{w}^t$& 客户端数据效用，服务器效益，社会总福利 \\
	$v$                  & 历史选择轮次,        \\
    $\textbf{w}^t, \textbf{w}^t$  & 全局模型，本地模型        \\

    ${\tau}^t, \tau_m^t$                 & 模型聚合权重        \\
	$Z, z_\text{max}^t, z_m$                  & 类别数目，类别最大数据量，数据类别数量      \\
    $\alpha$                  & DCGain的上限       \\
    $\Gamma(d_{z, m})$                  & 概率密度函数 \\
    $\lambda_m^t $                  & 无偏因子        \\
    $\varrho $                  & 模型大小        \\
    $\sigma$                  & 归一化因子        \\
    $\kappa_m^t $                  & 保证金        \\
    $\iota_m^t, \psi $    & ,控制UDQ曲线峰值位置的参数        \\
    $\tau $                  & 聚合权重       \\
    $\nu $                  & 控制DCGain曲线梯度的参数        \\
 
\end{notation}
